DynamicStereo: Consistent Dynamic Depth from Stereo Videos

We consider the problem of reconstructing a dynamic scene observed from a stereo camera. Most existing methods for depth from stereo treat different stereo frames independently, leading to temporally inconsistent depth predictions. Temporal consistency is especially important for immersive AR or VR scenarios, where flickering greatly diminishes the user experience. We propose DynamicStereo, a novel transformer-based architecture to estimate disparity for stereo videos. The network learns to pool information from neighboring frames to improve the temporal consistency of its predictions. Our architecture is designed to process stereo videos efficiently through divided attention layers. We also introduce Dynamic Replica, a new benchmark dataset containing synthetic videos of people and animals in scanned environments, which provides complementary training and evaluation data for dynamic stereo closer to real applications than existing datasets. Training with this dataset further improves the quality of predictions of our proposed DynamicStereo as well as prior methods. Finally, it acts as a benchmark for consistent stereo methods.

==> tab_dataset_comparison_extended.tex <==
\setlength\tabcolsep{.15em}
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{ llccccccccc }
\toprule
\multirow{2}{*}{Mtd} & \multirow{2}{*}{Data} & \multirow{2}{*}{KITTI} & \multicolumn{3}{c}{Middlebury} & \multirow{2}{*}{ETH3D} & \multicolumn{2}{c}{Sintel Stereo} & DR \\
\cmidrule(lr){4-6}
& & & full & half & quarter & & Clean & Final & full \\
\midrule
\multirow{2}{*}{[22]} & SF & \textbf{5.55} & 17.76 & 12.80 & 9.64 & 3.05 & \textbf{5.89} & 9.20 & 4.01\\
& (DR\&SF)/2 & 5.63 & \textbf{15.08} & \textbf{10.36} & \textbf{9.24} & \textbf{3.02} & 5.96 & \textbf{9.12} & \textbf{2.20}\\
\midrule
\multirow{2}{*}{[17]} & SF & 6.22 & 23.95 & 15.64 & 10.50 & 3.95 & 7.51 & 11.01 & 6.59 \\
 & (DR\&SF)/2 & \textbf{5.35} & \textbf{22.02} & \textbf{13.69} & \textbf{8.96} & \textbf{3.53} & \textbf{6.96} & \textbf{9.98} & \textbf{3.49} \\
\midrule
\end{tabular}
\vspace{-1em}
\caption{\textbf{Generalization.} We average across 3 runs with different seeds. EPE with a 3px threshold for KITTI 2015 and Sintel Stereo, 2px for Middlebury, 1px for ETH3D and our proposed DR.}%
\label{tab:tab_dataset_comparison_extended}
\end{table}

==> tab_inference_mode.tex <==
\setlength\tabcolsep{.4em}
\begin{table}[t]
\centering

\begin{tabular}{ cccccc}
\toprule
\multirow{2}{*}{Overlap} & \multirow{2}{*}{Window} & \multicolumn{2}{c}{Sintel Clean} & \multicolumn{2}{c}{Dynamic Replica}  \\
& & $\delta^t_{3px}$ & TEPE & $\delta^t_{1px}$ & TEPE  \\
\midrule
\xmark & 20 & 5.78 &  0.78  & 3.26 & 0.093 \\
\xmark & 12 & \textbf{5.76} & 0.78 & \textbf{3.16} & 0.111 \\
\cmark & 20  & 5.77 & \textbf{0.76}  & 3.32 & \textbf{0.075} \\
\cmark & 12  & \textbf{5.76} & 0.77 & 3.31 & 0.094 \\
\bottomrule
\end{tabular}

\caption{\textbf{Sliding Window Evaluation.} We evaluate the performance when varying the temporal window-size and overlap during evaluation. \todo{How much overlap is overlap?} half of the sliding window. We discard the second half of the first overlap and the first half of the second. For example, for a sequence of 30 frames, we run 20+20 (overlap 10)}
\label{tab:inference_mode}
\end{table}


==> tab_sota_comparison.tex <==
\setlength\tabcolsep{.4em}
\begin{table}[b]
\centering
\resizebox{1.\columnwidth}{!}
{
\begin{tabular}{ cl|cc|cc|cc}
\toprule
\multirow{3}{*}{Training data} & \multirow{3}{*}{Method} & \multicolumn{4}{c}{Sintel Stereo} & \multicolumn{2}{c}{Dynamic Replica} \\
& & \multicolumn{2}{c}{Clean} & \multicolumn{2}{c}{Final} & & \\
& & $\delta_{3px}$ & TEPE & $\delta_{3px}$ & TEPE & $\delta_{1px}$ & TEPE \\
\midrule
\multirow{3}{*}{SF}
& CODD (Li~\etal) & 8.68 & 1.44 & 17.46 & 2.32 & 6.59 & 0.105 \\ 
& RAFT Stereo & 6.12 & 0.92 & 10.4 & 2.10 & 5.51 & 0.145 \\

& Ours & \textbf{6.10} & \textbf{0.77} & \textbf{8.97} & \textbf{1.45} & \textbf{3.44} & \textbf{0.087} \\
\midrule
\multirow{2}{*}{DR+SF} & RAFT Stereo & \textbf{5.71} & 0.84 & 9.16 & 2.27 & \textbf{1.89} & \textbf{0.075} \\
& Ours & 5.77 & \textbf{0.76} & \textbf{8.68} & \textbf{1.42} & 3.32 & \textbf{0.075} \\
\midrule
SF+M+K &  CODD (Li~\etal) & 9.11 & 1.33 & 11.90  & 2.01 & 10.03 & 0.152 \\
SF+M & RAFT Stereo & 5.86 & 0.85 & \textbf{8.47} & 1.63 & 3.46 & 0.114 \\
7 datasets (incl. Sintel) & CRE Stereo & \textcolor{gray}{4.58} & \textcolor{gray}{0.67} & \textcolor{gray}{8.17} & \textcolor{gray}{1.90} & \textbf{1.75} & 0.088 \\

DR+SF & Ours & \textbf{5.77} & \textbf{0.76} & 8.68 & \textbf{1.42} & 3.32 & \textbf{0.075}  \\
\midrule
\end{tabular}}\vspace{-1em}
\caption{\textbf{Accuracy and Temporal consistency}. EPE with the standard $3$px threshold for Sintel and $1$px for Dynamic~Replica.}\label{tab:sota_comparison}
\end{table}
